Probabilistic Data Analysis with Probabilistic Programming

Probabilistic techniques are central to data analysis, but different approaches can be difficult to apply, combine, and compare. This paper introduces composable generative population models (CGPMs), a computational abstraction that extends directed graphical models and can be used to describe and compose a broad class of probabilistic data analysis techniques. Examples include hierarchical Bayesian models, multivariate kernel methods, discriminative machine learning, clustering algorithms, dimensionality reduction, and arbitrary probabilistic programs. We also demonstrate the integration of CGPMs into BayesDB, a probabilistic programming platform that can express data analysis tasks using a modeling language and a structured query language. The practical value is illustrated in two ways. First, CGPMs are used in an analysis that identifies satellite data records which probably violate Kepler's Third Law, by composing causal probabilistic programs with non-parametric Bayes in under 50 lines of probabilistic code. Second, for several representative data analysis tasks, we report on lines of code and accuracy measurements of various CGPMs, plus comparisons with standard baseline solutions from Python and MATLAB libraries.

==> tex/frontmatter/frontmatter.tex <==
% \documentclass[twoside,11pt]{article}
% \usepackage{jmlr2e}

% % Any additional packages needed should be included after jmlr2e.
% % Note that jmlr2e.sty includes epsfig, amssymb, natbib and graphicx,
% % and defines many common macros, such as 'proof' and 'example'.
% %
% % It also sets the bibliographystyle to plainnat; for more information on
% % natbib citation styles, see the natbib documentation, a copy of which
% % is archived at http://www.jmlr.org/format/natbib.pdf

% \usepackage{afterpage}
% \usepackage{newtxtext}
% \usepackage{textcomp}

% \begin{document}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\thispagestyle{empty}

\begin{center}
\large

\textbf{\LARGE Probabilistic Data Analysis with\\Probabilistic Programming}\\
\bigskip
by\\
\bigskip
{\Large Feras Ahmad Khaled Saad}\\
\bigskip
S.B., Electrical Engineering and Computer Science, M.I.T. (2016)\\
\bigskip
Submitted to the\\
Department of Electrical Engineering and Computer Science\\
in Partial Fulfillment of the Requirements for the Degree of\\
\bigskip
Master of Engineering in Electrical Engineering and Computer Science\\
\bigskip
at the\\
\bigskip
Massachusetts Institute of Technology\\
\bigskip
September 2016\\
\bigskip
\textcopyright \thinspace  2016 Massachusetts Institute of Technology.
    All rights reserved.\\
\end{center}

\vfill

\begin{center}
Signature of Author: \dotfill

\hfill Department of Electrical Engineering and Computer Science\\
\hfill September 21, 2016
\bigskip\bigskip\bigskip\bigskip

Certified by: \dotfill

\hfill Dr. Vikash Mansinghka\\
\hfill Research Scientist, Thesis Supervisor
\bigskip\bigskip\bigskip\bigskip

Accepted by: \dotfill

\hfill Dr. Christopher Terman\\
\hfill Chairman, Master of Engineering Thesis Committee
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage\phantom{h}
\thispagestyle{empty}

\newpage\phantom{h}

\begin{center}
\textbf{\LARGE Probabilistic Data Analysis with\\Probabilistic Programming}\\
\bigskip
by\\
\bigskip
{\Large Feras Ahmad Khaled Saad}\\
\bigskip
S.B., Electrical Engineering and Computer Science, M.I.T. (2016)\\
\bigskip
Submitted to the\\
Department of Electrical Engineering and Computer Science\\
in Partial Fulfillment of the Requirements for the Degree of\\
\bigskip
Master of Engineering in Electrical Engineering and Computer Science\\
\end{center}

\bigskip

\input{tex/abstract/abstract}

\bigskip

\noindent
Thesis Supervisor: Vikash Mansinghka\\
Title: Research Scientist

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage\phantom{h}

\begin{center}
\textit{To my mother and father, who gave and give me everything.}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage\phantom{h}

\section*{Acknowledgments}

This project would not be possible without the help of my friends and colleagues at the Probabilistic Computing Project.
I extend my sincerest gratitude to our principal investigator Vikash Mansinghka, the ideal professional and personal mentor in all respects.
I am grateful to DARPA for funding this research and my appointment as a research assistant through the Probabilistic Programming for Advanced Machine Learning program.

I thank my brother, Khaled, for his uplifting support, affection, and tolerance and engagement with my most atypical of thoughts.


==> tex/integrate-bayesdb/lst-mml-pop.tex <==
%!TEX root = ../../thesis.tex
\begin{figure}[t]

    \centering

    \begin{subfigure}[b]{.5\textwidth}
        \includegraphics[width=\textwidth]{figures/mml-template-population.pdf}
        \caption{Population Schema}
        \label{fig:mml-template-population}
    \end{subfigure}%
    \begin{subfigure}[b]{.5\textwidth}
        \includegraphics[width=\textwidth]{figures/mml-template-metamodel.pdf}
        \caption{Metamodel Schema}
        \label{fig:mml-template-metamodel}
    \end{subfigure}

    \bcaption{Metamodeling Language templates for population and
    metamodel schemas.}{%
    \subref{fig:mml-template-population} The population
    schema declares the list of variables and their statistical types.
    \subref{fig:mml-template-metamodel} The metamodel schema builds a
    network of composable generative population models; each CGPM is
    responsible for a subset of the variables and together they model the entire
    population.}
    \label{fig:mml-template}
\end{figure}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=2pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=3pt,
below right=5pt and 0pt of #1.south west] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


